High-order accurate schemes for Maxwell's equations with nonlinear active media and material interfaces

We describe a fourth-order accurate finite-difference time-domain scheme for solving dispersive Maxwell's equations with nonlinear multi-level carrier kinetics models. The scheme is based on an efficient single-step three time-level modified equation approach for Maxwell's equations in second-order form for the electric field coupled to ODEs for the polarization vectors and population densities of the atomic levels. The resulting scheme has a large CFL-one time-step. Curved interfaces between different materials are accurately treated with curvilinear grids and compatibility conditions. A novel hierarchical modified equation approach leads to an explicit scheme that does not require any nonlinear iterations. The hierarchical approach at interfaces leads to local updates at the interface with no coupling in the tangential directions. Complex geometry is treated with overset grids. Numerical stability is maintained using high-order upwind dissipation designed for Maxwell's equations in second-order form. The scheme is carefully verified for a number of two and three-dimensional problems. The resulting numerical model with generalized dispersion and arbitrary nonlinear multi-level system can be used for many plasmonic applications such as for ab initio time domain modeling of nonlinear engineered materials for nanolasing applications, where nano-patterned plasmonic dispersive arrays are used to enhance otherwise weak nonlinearity in the active media.

==> tex/diskArray.tex <==
\subsection{Array of MLA disks}\label{sec:diskArray}

% \subsection{A soliton solution in the single material}

In this section, we consider scattering of a Gaussian plane wave from an array of MLA disks...

Material file \texttt{mlaMat4levels.txt}.

\plotTwoFigsByWidth{fig/fourDiskMLAEfieldNormt1p0}{fig/fourDiskMLAPyt1p0}{Four MLA disks: computed solution. Left: $\| \Ev\|$. Right: $P_y$.}{fig:4diskArray}{7cm}

% \plotTwoFigsByWidth{fig/64DiskMLAEfieldNormt10}{fig/64DiskMLAPyt10}{Sixty-four MLA disks: computed solution. Left: $\| \Ev\|$. Right: $P_y$.}{fig:64diskArray}{7cm}

\plotThreeMatlabFigs{fig/64DiskMLAEfieldNormt10}{fig/64DiskMLAPyt10}{fig/64DiskMLAN0t10}{Sixty-four MLA disks: $\| \Ev\|$, $P_y$ and $N_0$}{fig:64diskArray}






==> tex/diskFig.tex <==
\clearpage
\section{Figure test}

Add a colour bar to a figure.

FIX ME: Colour bar bounds.

% ========================================
{% -----------------
% --------- START drawContour -----------
\newcommand{\drawContour}[7]{%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{fig/#2}{\figWidtha}};
  \draw(.55,.3) node[draw,fill=white,anchor=west,xshift=-1pt,yshift=7pt] {\scriptsize #3};
 % colour bar:
\begin{scope}[xshift=5pt,yshift=-12pt]
  \draw (\xcb,\ycb) node[anchor=south west,xshift=0.25cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
  \draw ( .8,0) node[anchor=north,xshift=+3pt,yshift=+7pt] {\scriptsize $#6$};
  \draw (4.8,0) node[anchor=north,xshift=+0pt,yshift=+7pt] {\scriptsize $#7$};
\end{scope}
\end{scope}
}
% --------- END drawContour -----------
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{4cm}% colour bar height
\newcommand{\xcb}{.5cm}% colour bar lower left corner
\newcommand{\ycb}{-.0cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*\real{.5}}% colour bar top label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
% ========================= DRAW ================
%
%%\newcommand{\figWidth}{8cm}
%%\newcommand{\trimfig}[2]{\trimhb{#1}{#2}{.0}{.0}{.0}{.0}}
\newcommand{\figWidtha}{5.25cm}
\newcommand{\trimfiga}[2]{\trimwb{#1}{#2}{.0}{.0}{.0}{.0}}
\begin{figure}[htb]
\begin{center}
\resizebox{16cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  \useasboundingbox (.25,.25) rectangle (18.,5.75);  % set the bounding box (so we have less surrounding white space)
  % \draw(-3,2) node[anchor=south west,xshift=-4pt,yshift=-1pt] {\trimfig{fig/dielectricDiskGDM}{\figWidth}};
  %
   \drawContour{xshift= 0.6cm,yshift=0.0cm}{oneDiskMLAEfieldNormt2}{$|\Ev|$ $t=2$}{$\Ev$}{$t=1.0$}{$0.0$}{$1.0$};
   \drawContour{xshift= 6.5cm,yshift=0.0cm}{oneDiskMLAPyt2}{$P_y$ $t=2$}{$p$}{$t=1.0$}{$0.0$}{$1.0$};
   \drawContour{xshift=12.2cm,yshift=0.0cm}{oneDiskMLAN3t2}{$N_3$ $t=2$}{$p$}{$t=1.0$}{$0.0$}{$1.06$};
% 
  %- \drawContour{xshift= 0.6cm,yshift=0cm}{multiDisk4aEnormt3}{$|\Ev|$ $t=3$}{$\Ev$}{$t=1.0$}{$0.0$}{$1.20$};
  %- \drawContour{xshift= 6.0cm,yshift=0cm}{multiDisk4aEnormt4}{$|\Ev|$ $t=4$}{$p$}{$t=1.0$}{$0.0$}{$0.99$};
  %- \drawContour{xshift=11.4cm,yshift=0cm}{multiDisk4aEnormt5}{$|\Ev|$ $t=5$}{$p$}{$t=1.0$}{$0.0$}{$0.93$};
% 
    %  --- AXES ON LOWER  LEFT FIG
    % \begin{scope}[xshift=1cm,yshift=0cm]
    %    \draw[|-|,very thick,xshift=-4pt,yshift=3pt] (0,0.12) node[anchor=east] {\scriptsize $-3$} -- (0,4) node[anchor=east] {\scriptsize $3$}; 
    %    \draw[|-|,very thick,yshift=1.25pt] (0.07,0.0) node[anchor=north] {\scriptsize $-4$} -- (5.23,0) node[anchor=north,xshift=-3pt] {\scriptsize $4$}; 
    % \end{scope}


% grid:
 \draw[step=1cm,gray] (1,0) grid (18,5.75);
\end{tikzpicture}
 }% end resize box
\end{center}
\caption{One MLA disk: $\| \Ev\|$, $P_y$ and $N_3$ at $t=2.0$.
  % A Gaussian traveling-wave scattering from the multi-disk structure. Contours of $|\Ev|$ at selected times.
  % the solution at $t=0.3$ on grid $\Gcd^{(8)}$.
   }
  \label{fig:oneDiskSolution}
\end{figure}
}


==> tex/mlaUpdateAlgorithmOrder2.tex <==
\section{Maxwell-MLA time-stepping algorithm, second-order accuracy}

\begin{Verbatim}[fontsize=\footnotesize]
! **********************************************************************************
! Macro updateMultilevelAtomic (MLA)
!
! **********************************************************************************
#beginMacro updateMultilevelAtomic(DIM,ORDER,GRIDTYPE)

  if( t.le.3*dt )then
    INFO("update-MULTI-LEVEL-ATOMIC_dim=DIM _order=ORDER _gridType=GRIDTYPE ***123***");
  end if
  
  ! initialize forcing functions
  fe=0.
  fet = 0.
  fett = 0.
  lapfe = 0.
  do iv=0,numberOfPolarizationVectors-1
    betav(iv) = 1./( 1.+.5*dt*b1v(iv) ) ! coefficients
    fpv(iv)=0.  ! initialize if not used
    fptv(iv)=0. 
    fpttv(iv)=0. 
    lapfpv(iv)=0.
  end do

  ! index location for first TZ nonlinear variable: 
  nce = pxc+nd*numberOfPolarizationVectors
  ! write(*,'(" *** UpadateMLA: pxc=",i2," numberOfPolarizationVectors=",i4," nce=",i4)') pxc,numberOfPolarizationVectors,nce 

  ! loop over space
  beginLoopsMask(i1,i2,i3,n1a,n1b,n2a,n2b,n3a,n3b)
  #If #ORDER eq "2"
    do m=0,nd-1
      pc=pxc+m
      ec=ex+m

      if( addForcing.ne.0 )then
        getEPMLAForcing(ec,pc) ! forcing functions for E and P
      end if

      ! ping old values
      ev = u(i1,i2,i3,ec)
      evm=um(i1,i2,i3,ec)
      do iv=0,numberOfPolarizationVectors-1
        pv(iv) = p(i1,i2,i3,m+iv*nd)
        pvm(iv)=pm(i1,i2,i3,m+iv*nd)
      end do

      ! write(*,*) 'Inside updateDispersive'

      ! write(*,*) 'Inside updateDispersive order=2'
      
      ! get laplacians
      #If #DIM eq "2"
          #If #GRIDTYPE eq "rectangular"

            ! INFO("FD22r-2D-dispersive-Any-PV");
            ! write(*,*) 'Inside updateDispersive rectangular order=2'

            ! elap2 = ulaplacian22r(i1,i2,i3,ec)
            elap2 = lap2d2(i1,i2,i3,ec)

          #Elif #GRIDTYPE eq "curvilinear"

            ! INFO("FD22c-2D-dispersive-any-PV");

            ! write(*,*) 'Inside updateDispersive curvilinear order=2'

            elap2 = ulaplacian22(i1,i2,i3,ec)

          #End


      #Elif #DIM eq "3"
          #If #GRIDTYPE eq "rectangular"

            ! INFO("FD22r-3D-dispersive-Any-PV");

            elap2 = lap3d2(i1,i2,i3,ec)

          #Elif #GRIDTYPE eq "curvilinear"

            ! INFO("FD22c-3D-dispersive-any-PV");

            elap2 = ulaplacian23(i1,i2,i3,ec)

          #End

      #Else
          ! Stop message
          stop 123
      #End

      ! second order update of P_m
      pSum = 0.
      do iv=0,numberOfPolarizationVectors-1

        pvn(iv) = 2.*pv(iv)-pvm(iv) + 0.5*dt*b1v(iv)*pvm(iv) - dtsq*b0v(iv)*pv(iv) + dtsq*fpv(iv)

        do na = 0,numberOfAtomicLevels-1 ! \Delta N^n*E^n
          pvn(iv) = pvn(iv) + dtsq*pnec(iv,na)*q(i1,i2,i3,na)*ev
        enddo

        pn(i1,i2,i3,m+iv*nd) = betav(iv)*pvn(iv)

        pSum = pSum + betav(iv)*pvn(iv) -2.*pv(iv) + pvm(iv)

      end do
      
      ! second order update of E
      evn = (2.*ev-evm) + csq*dtsq*elap2 - alphaP*pSum + dtsq*fe
      un(i1,i2,i3,ec) = evn

      ! End of second order code
    end do !m=0,nd-1 over space dim

    ! outside of dimension loop
    ! E(t+dt) and P(t+dt) are now known 
    ! --- second order update of N ---
    ! MLA
    do na=0,numberOfAtomicLevels-1
      ! forcing function
      getMLAForcing(na)
    enddo
    ! N_t
    do na=0,numberOfAtomicLevels-1
      ! first time derivative
      qt(na) = fnv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qt(na) = qt(na)+prc(na,iv)*q(i1,i2,i3,iv) 
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qt(na) = qt(na)+peptc(na,iv)*u(i1,i2,i3,m)*(pn(i1,i2,i3,m+iv*nd)-pm(i1,i2,i3,m+iv*nd))/(2.*dt)
        enddo
      enddo
    enddo
    ! N_tt
    do na=0,numberOfAtomicLevels-1
      qtt(na) = fntv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qtt(na) = qtt(na)+prc(na,iv)*qt(iv)
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qtt(na) = qtt(na)+peptc(na,iv)*(un(i1,i2,i3,m)-um(i1,i2,i3,m))/(2.*dt)*(pn(i1,i2,i3,m+iv*nd)-pm(i1,i2,i3,m+iv*nd))/(2.0*dt) \
                           +peptc(na,iv)*u(i1,i2,i3,m)*(pn(i1,i2,i3,m+iv*nd)-2.0*p(i1,i2,i3,m+iv*nd)+pm(i1,i2,i3,m+iv*nd))/dtsq
        enddo
      enddo
    enddo

    ! fill in the population densities "N"
    do na=0,numberOfAtomicLevels-1
      qn(i1,i2,i3,na) = q(i1,i2,i3,na) + dt*qt(na) + dt**2/2.*qtt(na)
    end do


  #Else
    ! Stop message if order not 2 or 4
    stop 123
  #End

  endLoopsMask()

#endMacro
\end{Verbatim}

==> tex/mlaUpdateAlgorithmOrder4.tex <==
\section{Maxwell-MLA time-stepping algorithm, fourth-order accuracy}

\begin{Verbatim}[fontsize=\footnotesize]
! **********************************************************************************
! Macro updateMultilevelAtomic (MLA)
!
! Initial version: July 2020
!
! **********************************************************************************
#beginMacro updateMultilevelAtomic(DIM,ORDER,GRIDTYPE)

  if( t.le.3*dt )then
    INFO("update-MULTI-LEVEL-ATOMIC_dim=DIM _order=ORDER _gridType=GRIDTYPE ***123***");
  end if
  
  ! initialize forcing functions
  fe=0.
  fet = 0.
  fett = 0.
  lapfe = 0.
  do iv=0,numberOfPolarizationVectors-1
    betav(iv) = 1./( 1.+.5*dt*b1v(iv) ) ! coefficients
    fpv(iv)=0.  ! initialize if not used
    fptv(iv)=0. 
    fpttv(iv)=0. 
    lapfpv(iv)=0.
  end do

  ! index location for first TZ nonlinear variable: 
  nce = pxc+nd*numberOfPolarizationVectors
  ! write(*,'(" *** UpadateMLA: pxc=",i2," numberOfPolarizationVectors=",i4," nce=",i4)') pxc,numberOfPolarizationVectors,nce 

  ! loop over space
  beginLoopsMask(i1,i2,i3,n1a,n1b,n2a,n2b,n3a,n3b)
  #If #ORDER eq "2"
    do m=0,nd-1
      pc=pxc+m
      ec=ex+m

      if( addForcing.ne.0 )then
        getEPMLAForcing(ec,pc) ! forcing functions for E and P
      end if

      ! ping old values
      ev = u(i1,i2,i3,ec)
      evm=um(i1,i2,i3,ec)
      do iv=0,numberOfPolarizationVectors-1
        pv(iv) = p(i1,i2,i3,m+iv*nd)
        pvm(iv)=pm(i1,i2,i3,m+iv*nd)
      end do

      ! write(*,*) 'Inside updateDispersive'

      ! write(*,*) 'Inside updateDispersive order=2'
      
      ! get laplacians
      #If #DIM eq "2"
          #If #GRIDTYPE eq "rectangular"

            ! INFO("FD22r-2D-dispersive-Any-PV");
            ! write(*,*) 'Inside updateDispersive rectangular order=2'

            ! elap2 = ulaplacian22r(i1,i2,i3,ec)
            elap2 = lap2d2(i1,i2,i3,ec)

          #Elif #GRIDTYPE eq "curvilinear"

            ! INFO("FD22c-2D-dispersive-any-PV");

            ! write(*,*) 'Inside updateDispersive curvilinear order=2'

            elap2 = ulaplacian22(i1,i2,i3,ec)

          #End


      #Elif #DIM eq "3"
          #If #GRIDTYPE eq "rectangular"

            ! INFO("FD22r-3D-dispersive-Any-PV");

            elap2 = lap3d2(i1,i2,i3,ec)

          #Elif #GRIDTYPE eq "curvilinear"

            ! INFO("FD22c-3D-dispersive-any-PV");

            elap2 = ulaplacian23(i1,i2,i3,ec)

          #End

      #Else
          ! Stop message
          stop 123
      #End

      ! second order update of P_m
      pSum = 0.
      do iv=0,numberOfPolarizationVectors-1

        pvn(iv) = 2.*pv(iv)-pvm(iv) + 0.5*dt*b1v(iv)*pvm(iv) - dtsq*b0v(iv)*pv(iv) + dtsq*fpv(iv)

        do na = 0,numberOfAtomicLevels-1 ! \Delta N^n*E^n
          pvn(iv) = pvn(iv) + dtsq*pnec(iv,na)*q(i1,i2,i3,na)*ev
        enddo

        pn(i1,i2,i3,m+iv*nd) = betav(iv)*pvn(iv)

        pSum = pSum + betav(iv)*pvn(iv) -2.*pv(iv) + pvm(iv)

      end do
      
      ! second order update of E
      evn = (2.*ev-evm) + csq*dtsq*elap2 - alphaP*pSum + dtsq*fe
      un(i1,i2,i3,ec) = evn

      ! End of second order code
    end do !m=0,nd-1 over space dim

    ! outside of dimension loop
    ! E(t+dt) and P(t+dt) are now known 
    ! --- second order update of N ---
    ! MLA
    do na=0,numberOfAtomicLevels-1
      ! forcing function
      getMLAForcing(na)
    enddo
    ! N_t
    do na=0,numberOfAtomicLevels-1
      ! first time derivative
      qt(na) = fnv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qt(na) = qt(na)+prc(na,iv)*q(i1,i2,i3,iv) 
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qt(na) = qt(na)+peptc(na,iv)*u(i1,i2,i3,m)*(pn(i1,i2,i3,m+iv*nd)-pm(i1,i2,i3,m+iv*nd))/(2.*dt)
        enddo
      enddo
    enddo
    ! N_tt
    do na=0,numberOfAtomicLevels-1
      qtt(na) = fntv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qtt(na) = qtt(na)+prc(na,iv)*qt(iv)
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qtt(na) = qtt(na)+peptc(na,iv)*(un(i1,i2,i3,m)-um(i1,i2,i3,m))/(2.*dt)*(pn(i1,i2,i3,m+iv*nd)-pm(i1,i2,i3,m+iv*nd))/(2.0*dt) \
                           +peptc(na,iv)*u(i1,i2,i3,m)*(pn(i1,i2,i3,m+iv*nd)-2.0*p(i1,i2,i3,m+iv*nd)+pm(i1,i2,i3,m+iv*nd))/dtsq
        enddo
      enddo
    enddo

    ! fill in the population densities "N"
    do na=0,numberOfAtomicLevels-1
      qn(i1,i2,i3,na) = q(i1,i2,i3,na) + dt*qt(na) + dt**2/2.*qtt(na)
    end do

  #Elif #ORDER eq '4'
    !
    ! second order predictions
    !
    do m=0,nd-1
      pc=pxc+m
      ec=ex+m

      if ( addForcing.ne.0) then 
        getEPMLAForcing(ec,pc) ! forcing functions for E and P
      end if

      ! ping old values
      ev = u(i1,i2,i3,ec)
      evm=um(i1,i2,i3,ec)
      do iv=0,numberOfPolarizationVectors-1
        pv(iv) = p(i1,i2,i3,m+iv*nd)
        pvm(iv)=pm(i1,i2,i3,m+iv*nd)
      end do

      ! get laplacians
      #If #DIM eq "2"
          #If #GRIDTYPE eq "rectangular"

            ! INFO("FD22r-2D-dispersive-Any-PV");
            ! write(*,*) 'Inside updateDispersive rectangular order=2'

            elap2 = lap2d2(i1,i2,i3,ec)

          #Elif #GRIDTYPE eq "curvilinear"

            ! INFO("FD22c-2D-dispersive-any-PV");
            ! write(*,*) 'Inside updateDispersive curvilinear order=2'

            elap2 = ulaplacian22(i1,i2,i3,ec)

          #End

      #Elif #DIM eq "3"
          #If #GRIDTYPE eq "rectangular"

            ! INFO("FD22r-3D-dispersive-Any-PV");

            elap2 = lap3d2(i1,i2,i3,ec)

          #Elif #GRIDTYPE eq "curvilinear"

            ! INFO("FD22c-3D-dispersive-any-PV");

            elap2 = ulaplacian23(i1,i2,i3,ec)

          #End

      #Else
          ! Stop message
          stop 123
      #End

      ! second order update of P_m
      pSum = 0.
      do iv=0,numberOfPolarizationVectors-1

        pvn(iv) = 2.*pv(iv)-pvm(iv) + 0.5*dt*b1v(iv)*pvm(iv) - dtsq*b0v(iv)*pv(iv) + dtsq*fpv(iv)

        do na = 0,numberOfAtomicLevels-1 ! \Delta N^n*E^n
          pvn(iv) = pvn(iv) + dtsq*pnec(iv,na)*q(i1,i2,i3,na)*ev
        enddo

        pn(i1,i2,i3,m+iv*nd) = betav(iv)*pvn(iv)

        pSum = pSum + betav(iv)*pvn(iv) -2.*pv(iv) + pvm(iv)

      end do
      
      ! second order update of E
      evn = (2.*ev-evm) + csq*dtsq*elap2 - alphaP*pSum + dtsq*fe
      un(i1,i2,i3,ec) = evn

      ! End of second order code
    end do ! m=0,nd-1 over space dim

    ! outside of dimension loop
    ! --- second order update of N ---
    ! MLA
    do na=0,numberOfAtomicLevels-1
      ! forcing functions for both the second order codes and fourth order codes
      getMLAForcing44(na)
    enddo
    ! N_t
    do na=0,numberOfAtomicLevels-1
      qt(na) = fnv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qt(na) = qt(na)+prc(na,iv)*q(i1,i2,i3,iv) 
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qt(na) = qt(na)+peptc(na,iv)*u(i1,i2,i3,m)*(pn(i1,i2,i3,m+iv*nd)-pm(i1,i2,i3,m+iv*nd))/(2.*dt)
        enddo
      enddo
    enddo
    ! N_tt
    do na=0,numberOfAtomicLevels-1
      qtt(na) = fntv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qtt(na) = qtt(na)+prc(na,iv)*qt(iv)
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qtt(na) = qtt(na)+peptc(na,iv)*(un(i1,i2,i3,m)-um(i1,i2,i3,m))/(2.*dt)*(pn(i1,i2,i3,m+iv*nd)-pm(i1,i2,i3,m+iv*nd))/(2.0*dt) \
                           +peptc(na,iv)*u(i1,i2,i3,m)*(pn(i1,i2,i3,m+iv*nd)-2.0*p(i1,i2,i3,m+iv*nd)+pm(i1,i2,i3,m+iv*nd))/dtsq
        enddo
      enddo
    enddo
    ! fill in the population densities "N"
    do na=0,numberOfAtomicLevels-1
      qn(i1,i2,i3,na) = q(i1,i2,i3,na) + dt*qt(na) + dt**2/2.*qtt(na)
    end do

    !----------------------
    ! fourth order update
    !----------------------
    ! write(*,*) 'Inside updateMultilevelAtomic 2D rectangular order=4'
    do m=0,nd-1 ! loop over dimension
      pc=pxc+m
      ec=ex+m

      if( addForcing.ne.0 )then
          getEPMLAForcing44(ec,pc)
      end if

      ! ping the current indexed values of E and P
      evn=un(i1,i2,i3,ec)
      ev = u(i1,i2,i3,ec)
      evm=um(i1,i2,i3,ec)

      do iv=0,numberOfPolarizationVectors-1
        pvn(iv)=pn(i1,i2,i3,m+iv*nd)
        pv(iv) = p(i1,i2,i3,m+iv*nd)
        pvm(iv)=pm(i1,i2,i3,m+iv*nd)
      end do

      ! write(*,*) 'Inside updateDispersive order=4'

      ! space derivatives of E, P, N
      #If #DIM eq "2"
        #If #GRIDTYPE eq "rectangular"

          ! INFO("FD44r-2D-dispersive-Any-PV");
          ! write(*,*) 'Inside updateDispersive 2D rectangular order=4'

          ! laplacians of E
          elap4   = lap2d4(i1,i2,i3,ec)
          elapsq2 = lap2d2Pow2(i1,i2,i3,ec)
          elap2   = lap2d2(i1,i2,i3,ec)
          elap2m  = lap2d2m(i1,i2,i3,ec)

          ! first order derivatives of E
          ex2v = ex2(i1,i2,i3,ec)
          ey2v = ey2(i1,i2,i3,ec)

          ! laplacians of P
          do iv=0,numberOfPolarizationVectors-1
            pxxv(iv)  = plap2d4(i1,i2,i3,m+iv*nd)
            pxxvm(iv) = plap2d4m(i1,i2,i3,m+iv*nd)
          end do

          
          do na=0,numberOfAtomicLevels-1
            qlap2(na) = qlap2d2(i1,i2,i3,na) ! laplacian of N
            qx2v(na) =  qx2(i1,i2,i3,na) ! first order derivatives of N
            qy2v(na) =  qy2(i1,i2,i3,na)
            ! chain rule for \Delta (E*N)
            qelap2(na) = ev*qlap2(na)+q(i1,i2,i3,na)*elap2+2.*ex2v*qx2v(na)+2.*ey2v*qy2v(na)
          enddo

        #Elif #GRIDTYPE eq "curvilinear"

          ! INFO("FD44c-2D-dispersive-any-PV");

          ! write(*,*) 'Inside updateDispersive 2D curvilinear order=4'

          ! laplacians of E
          elap4   = ulaplacian42(i1,i2,i3,ec)
          elapsq2 = vlaplacian22(i1,i2,i3,ec)
          elap2   = ulaplacian22(i1,i2,i3,ec)
          elap2m  = umlaplacian22(i1,i2,i3,ec)

          ! first order derivatives of E
          ex2v = ux22(i1,i2,i3,ec)
          ey2v = uy22(i1,i2,i3,ec)

          ! laplacians of P
          do iv=0,numberOfPolarizationVectors-1
            pxxv(iv)  = plaplacian42(i1,i2,i3,m+iv*nd)
            pxxvm(iv) = pmlaplacian42(i1,i2,i3,m+iv*nd)
          end do

          do na=0,numberOfAtomicLevels-1
            qlap2(na) = qlaplacian22(i1,i2,i3,na)
            qx2v(na) =  qx22(i1,i2,i3,na)
            qy2v(na) =  qy22(i1,i2,i3,na)
            ! chain rule for \Delta (E*N)
            qelap2(na) = ev*qlap2(na)+q(i1,i2,i3,na)*elap2+2.*ex2v*qx2v(na)+2.*ey2v*qy2v(na)
          enddo

        #End


      #Elif #DIM eq "3"
        #If #GRIDTYPE eq "rectangular"

          ! INFO("FD44r-3D-dispersive-Any-PV");
          ! write(*,*) 'Inside updateDispersive 3D rectangular order=4'
          
          ! laplacians of E
          elap4   = lap3d4(i1,i2,i3,ec)
          elapsq2 = lap3d2Pow2(i1,i2,i3,ec)
          elap2   = lap3d2(i1,i2,i3,ec)
          elap2m  = lap3d2m(i1,i2,i3,ec)

          ! first order derivatives of E
          ex2v = ex2(i1,i2,i3,ec)
          ey2v = ey2(i1,i2,i3,ec)
          ez2v = ez2(i1,i2,i3,ec)

          ! laplacians of P
          do iv=0,numberOfPolarizationVectors-1
            pxxv(iv)  = plap3d4(i1,i2,i3,m+iv*nd)
            pxxvm(iv) = plap3d4m(i1,i2,i3,m+iv*nd)
          end do

          do na=0,numberOfAtomicLevels-1
            qlap2(na) = qlap3d2(i1,i2,i3,na)
            qx2v(na) =  qx2(i1,i2,i3,na)
            qy2v(na) =  qy2(i1,i2,i3,na)
            qz2v(na) =  qz2(i1,i2,i3,na)
            ! chain rule for \Delta (E*N)
            qelap2(na) = ev*qlap2(na)+q(i1,i2,i3,na)*elap2+2.*ex2v*qx2v(na)+2.*ey2v*qy2v(na)+2.*ez2v*qz2v(na)
          enddo

        #Elif #GRIDTYPE eq "curvilinear"

          ! INFO("FD44c-3D-dispersive-any-PV");
          ! write(*,*) 'Inside updateDispersive 3D curvilinear order=4'

          ! laplacians of E
          elap4   = ulaplacian43(i1,i2,i3,ec)
          elapsq2 = vlaplacian23(i1,i2,i3,ec)
          elap2   = ulaplacian23(i1,i2,i3,ec)
          elap2m  = umlaplacian23(i1,i2,i3,ec)

          ! first order derivatives of E
          ex2v = ux23(i1,i2,i3,ec)
          ey2v = uy23(i1,i2,i3,ec)
          ez2v = uz23(i1,i2,i3,ec)

          ! laplacians of P
          do iv=0,numberOfPolarizationVectors-1
            pxxv(iv)   = plaplacian43(i1,i2,i3,m+iv*nd)
            pxxvm(iv) = pmlaplacian43(i1,i2,i3,m+iv*nd)
          end do

          do na=0,numberOfAtomicLevels-1
            qlap2(na) = qlaplacian23(i1,i2,i3,na)
            qx2v(na) =  qx23(i1,i2,i3,na)
            qy2v(na) =  qy23(i1,i2,i3,na)
            qz2v(na) =  qz23(i1,i2,i3,na)
            ! chain rule for \Delta (E*N)
            qelap2(na) = ev*qlap2(na)+q(i1,i2,i3,na)*elap2+2.*ex2v*qx2v(na)+2.*ey2v*qy2v(na)+2.*ez2v*qz2v(na)
          enddo

        #End
      #End

      !--------------------
      ! fourth order P
      !--------------------
      ! second order accurate terms
      et = (evn-evm)/(2.0*dt)
      ett = (evn-2.*ev+evm)/dtsq
      ptttSum = 0.
      do iv = 0,numberOfPolarizationVectors-1
        ptv(m,iv) = (pvn(iv)-pvm(iv))/(2.0*dt)
        pttv(m,iv) = (pvn(iv)-2.0*pv(iv)+pvm(iv))/dtsq
        ptttv(m,iv) = -b1v(iv)*pttv(m,iv)-b0v(iv)*ptv(m,iv)+fptv(iv)
        do na = 0,numberOfAtomicLevels-1 ! update using ODE
          ptttv(m,iv) = ptttv(m,iv) + pnec(iv,na)*qt(na)*ev \
                                    + pnec(iv,na)*q(i1,i2,i3,na)*et
        enddo
        pttttv(m,iv) = -b1v(iv)*ptttv(m,iv)-b0v(iv)*pttv(m,iv)+fpttv(iv) ! update using ODE
        do na = 0,numberOfAtomicLevels-1
          pttttv(m,iv) = pttttv(m,iv) + pnec(iv,na)*qtt(na)*ev \
                                   + 2.*pnec(iv,na)*qt(na)*et \
                                      + pnec(iv,na)*q(i1,i2,i3,na)*ett
        enddo
        ptttSum = ptttSum + ptttv(m,iv)
      enddo

      ! update 4th order accurate P
      pSum = 0.
      pxxSum = 0.
      do iv=0,numberOfPolarizationVectors-1

        pvn(iv) = 2.*pv(iv)-pvm(iv) + 0.5*dt*b1v(iv)*pvm(iv) + dt**4/12.*pttttv(m,iv) + dt**4/6.*b1v(iv)*ptttv(m,iv) - dtsq*b0v(iv)*pv(iv) + dtsq*fpv(iv)

        do na = 0,numberOfAtomicLevels-1 ! \Delta N^n*E^n
          pvn(iv) = pvn(iv) + dtsq*pnec(iv,na)*q(i1,i2,i3,na)*ev
        enddo

        pvn(iv) = betav(iv)*pvn(iv)

        pn(i1,i2,i3,m+iv*nd) = pvn(iv) ! store updated P

        pSum = pSum + pvn(iv) - 2.*pv(iv) + pvm(iv) ! sum P_tt

        ! laplacians of P^{n+1}
        pxxvn(iv) = 2.*pxxv(iv)-pxxvm(iv) + 0.5*dt*b1v(iv)*pxxvm(iv) - dtsq*b0v(iv)*pxxv(iv) + dtsq*lapfpv(iv)

        do na = 0,numberOfAtomicLevels-1 ! \Delta N^n*E^n
          pxxvn(iv) = pxxvn(iv) + dtsq*pnec(iv,na)*qelap2(na)
        enddo
        ! time derivatives of laplacian of P
        pxxSum = pxxSum + betav(iv)*pxxvn(iv) - 2.*pxxv(iv) + pxxvm(iv)

      end do

      !-------------------
      ! fourth order E
      !-------------------
      
      evn =   (2.*ev-evm) + csq*dtsq*elap4 - alphaP*pSum + dtsq*fe \
            + dt**4/12.*(csq**2*elapsq2 - alphaP*csq*pxxSum/dtsq + csq*lapfe + fett)
      
      ! store 4th order accurate E
      un(i1,i2,i3,ec) = evn

      ! laplacian of E at new time
      elap2n = 2.*elap2-elap2m+dtsq*csq*elapsq2-alphaP*pxxSum + dtsq*lapfe
      ettt = (csq*elap2n-csq*elap2m)/(2.0*dt)-alphaP*ptttSum + fet ! E_ttt
      
      ! store in (Ex,Ey,E_z)
      ettv(m) = (evn-2.*ev+evm)/dtsq
      etttv(m) = ettt

      ! fourth order accurate terms
      etv(m) = (evn-evm)/(2.*dt)-dtsq/6.*ettt
      do iv = 0,numberOfPolarizationVectors-1
        ptv(m,iv) = (pvn(iv)-pvm(iv))/(2.*dt)-dtsq/6.*ptttv(m,iv)
        pttv(m,iv) = -b1v(iv)*ptv(m,iv)-b0v(iv)*pv(iv) + fpv(iv)
        do na = 0,numberOfAtomicLevels-1
          pttv(m,iv) = pttv(m,iv) + pnec(iv,na)*q(i1,i2,i3,na)*ev
        enddo
        ! second order accurate terms
        ptttv(m,iv) = -b1v(iv)*pttv(m,iv)-b0v(iv)*ptv(m,iv)+fptv(iv)
        do na = 0,numberOfAtomicLevels-1
          ptttv(m,iv) = ptttv(m,iv) + pnec(iv,na)*qt(na)*ev \
                                     +pnec(iv,na)*q(i1,i2,i3,na)*etv(m)
        enddo
        pttttv(m,iv) = -b1v(iv)*ptttv(m,iv)-b0v(iv)*pttv(m,iv)+fpttv(iv)
        do na = 0,numberOfAtomicLevels-1
          pttttv(m,iv) = pttttv(m,iv) + pnec(iv,na)*qtt(na)*ev \
                                   +2.0*pnec(iv,na)*qt(na)*etv(m) \
                                      + pnec(iv,na)*q(i1,i2,i3,na)*ettv(m)
        enddo
      enddo 

    enddo ! m=0,nd-1
    
    !-------------------
    ! fourth order N
    !-------------------
    ! fourth order accurate terms
    ! N_t
    do na=0,numberOfAtomicLevels-1
      qt(na) = fnv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qt(na) = qt(na)+prc(na,iv)*q(i1,i2,i3,iv) 
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qt(na) = qt(na)+peptc(na,iv)*u(i1,i2,i3,m)*ptv(m,iv)
        enddo
      enddo
    enddo
    ! N_tt
    do na=0,numberOfAtomicLevels-1
      qtt(na) = fntv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qtt(na) = qtt(na)+prc(na,iv)*qt(iv)
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qtt(na) = qtt(na)+peptc(na,iv)*etv(m)*ptv(m,iv) \
                           +peptc(na,iv)*u(i1,i2,i3,m)*pttv(m,iv)
        enddo
      enddo
    enddo

    ! N_ttt
    do na=0,numberOfAtomicLevels-1
      qttt(na) = fnttv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qttt(na) = qttt(na)+prc(na,iv)*qtt(iv)
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qttt(na) = qttt(na)+peptc(na,iv)*ettv(m)*ptv(m,iv) \
                          +2.*peptc(na,iv)*etv(m)*pttv(m,iv) \
                             +peptc(na,iv)*u(i1,i2,i3,m)*ptttv(m,iv)
        enddo
      enddo
    enddo

    ! N_tttt
    do na=0,numberOfAtomicLevels-1
      qtttt(na) = fntttv(na)
      do iv=0,numberOfAtomicLevels-1 ! relaxation
        qtttt(na) = qtttt(na)+prc(na,iv)*qttt(iv)
      enddo
      do m=0,nd-1 ! dot product
        do iv = 0,numberOfPolarizationVectors-1 ! loop over pc
          qtttt(na) = qtttt(na)+peptc(na,iv)*etttv(m)*ptv(m,iv) \
                            +3.*peptc(na,iv)*ettv(m)*pttv(m,iv) \
                            +3.*peptc(na,iv)*etv(m)*ptttv(m,iv) \
                               +peptc(na,iv)*u(i1,i2,i3,m)*pttttv(m,iv)
        enddo
      enddo
    enddo

    do na=0,numberOfAtomicLevels-1
      qn(i1,i2,i3,na) = q(i1,i2,i3,na) + dt*qt(na) + dt**2/2.*qtt(na) + dt**3/6.*qttt(na) + dt**4/24.*qtttt(na)
    end do

  #Else
    ! Stop message if order not 2 or 4
    stop 123
  #End

  endLoopsMask()

#endMacro
\end{Verbatim}

==> tex/oneDiskTwoLayersEfieldNormS22.tex <==

% ================== TRIG TZ FOR AN MLA DISK ==========
{% ------ GRIDS ------
% --------- START drawContour -----------
\newcommand{\drawContour}[7]{%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfiga{fig/#2}{\figWidtha}};
  \draw(.75,.5) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #3};
 % colour bar:
\begin{scope}[xshift=-.1cm,yshift=-3pt]
  \draw (\xcb,\ycb) node[anchor=south west,xshift=0.25cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
  \draw (.8,0) node[anchor=north,xshift=+3pt,yshift=+2pt] {\scriptsize $#6$};
  \draw (4.8,0) node[anchor=north,xshift=+0pt,yshift=+2pt] {\scriptsize $#7$};
\end{scope}
\end{scope}
}
\newcommand{\drawContourC}[7]{%
\begin{scope}[#1]
\draw(0.0,0) node[anchor=south west,xshift=-4pt,yshift=+0pt] {\trimfigc{fig/#2}{\figWidth}};
  \draw(.75,.75) node[draw,fill=white,anchor=west,xshift=2pt,yshift=1pt] {\scriptsize #3};
 % colour bar:
\begin{scope}[xshift=-.1cm,yshift=-3pt]
  \draw (\xcb,\ycb) node[anchor=south west,xshift=0.25cm,yshift=.5cm,rotate=-90] {\trimfigcb{fig/colourBarLines}{\cbWidth}{\cbHeight}};
  \draw (.75,0) node[anchor=north,xshift=+3pt,yshift=+2pt] {\scriptsize $#6$};
  \draw (4.8,0) node[anchor=north,xshift=+0pt,yshift=+2pt] {\scriptsize $#7$};
\end{scope}
\end{scope}
}
% --------- END drawContour -----------
% -- for colour bar ----
\newcommand{\cbWidth}{.2cm}% colour bar width
\newcommand{\cbHeight}{4cm}% colour bar height
\newcommand{\xcb}{.5cm}% colour bar lower left corner
\newcommand{\ycb}{-.2cm}% colour bar lower left corner
\setlength{\ycbTop}{\ycb+\cbHeight}% colour bar top label position
\setlength{\ycbMid}{\ycb+\cbHeight*\real{.5}}% colour bar top label position
\newcommand{\trimfigcb}[3]{\includegraphics[width=#2, height=#3, clip, trim=17cm 2.35cm 1.65cm 2.35cm]{#1}}
%
% ========================= DRAW ================
%
% \def\rad{1.27}% .8 
% \newcommand{\plotDisk}{
% % Plot the rigid body
% \fill[fill=red!20,draw=red,line width=2pt] 
%       plot[samples=100, domain=0.:360] ( {\rad*cos(\x)} , {\rad*sin(\x)} ) -- cycle ;
% }
\newcommand{\figWidth}{5.cm}
\newcommand{\trimfig}[2]{\trimh{#1}{#2}{.02}{.02}{.02}{.02}}
\newcommand{\figWidtha}{5.75cm}
\newcommand{\trimfiga}[2]{\trimh{#1}{#2}{.04}{.12}{.07}{.09}}
\newcommand{\trimfigc}[2]{\trimh{#1}{#2}{.18}{.18}{.15}{.4}}
\begin{figure}[htb]
\begin{center}
\resizebox{8cm}{!}{% START resize box
\begin{tikzpicture}[scale=1]
  % \useasboundingbox (.4,0.2) rectangle (16.5,5.8);  % set the bounding box (so we have less surrounding white space)
  % \draw(0.25,0) node[anchor=south west,xshift=-4pt,yshift=-1pt] {\trimfig{fig/oneDiskMLAGridG2}{\figWidth}};
   % \drawContourC{xshift= 5.6cm,yshift=-.08cm}{curvedInterfaceG4EyT1p0}{$E_y$ $t=1.0$}{$\Ev$}{$t=0.3$}{$-0.5$}{$0.5$};
   \drawContourC{xshift=0.cm,yshift=0.cm}{oneDiskTwoLayersMlaEfieldNormS22O4G8}{$||\bm{E}||$ at $t=4.2$}{$p$}{$t=0.3$}{$0$}{$1.04325$};
   % \drawContour{xshift= 5.6cm,yshift=-.08cm}{oneDiskMLA3Eyt1p0}{$E_y$ $t=1.0$}{$\Ev$}{$t=0.3$}{$-0.5$}{$0.5$};
   % \drawContour{xshift=11.5cm,yshift=-.08cm}{oneDiskMLA3EyErrt1p0}{$E_y$-error  $t=1.0$}{$p$}{$t=0.3$}{$??$}{$??$};
   %\drawContour{xshift=11.2cm,yshift=-.08cm}{oneDiskMLA3Eyt0p3}{$P_y$}{$p$}{$t=0.3$}{$??$}{$??$};

  %
  % \begin{scope}[xshift=.6cm,yshift=.05cm]
  %    \draw[|-|,very thick,xshift=-4pt] (0,0.1) node[anchor=east] {\footnotesize $-1$} -- (0,5.1) node[anchor=east] {\footnotesize $1$}; 
  %    \draw[|-|,very thick,yshift=-3pt] (0.08,0.0) node[anchor=north] {\footnotesize $-1$} -- (5.1,0) node[anchor=north,xshift=-3pt] {\footnotesize $1$}; 

  %    \begin{scope}[xshift=1.8pt,yshift=1.95pt]
  %      \draw[very thick] (2.5cm,2.5cm) circle(1.3cm);
  %      \draw[->,thick,xshift=2.5cm,yshift=2.5cm] (0,0) -- (.91,.91) node[anchor=east] {\scriptsize $r_d$};
  %     \end{scope}
  % \end{scope}

  %
  
% \drawContour{xshift=5.6cm,yshift=0cm}{diskEigExt1p0}{$E_x$}{$\Ev$}{$t=1.0$}{$-.18$}{$.18$};
% \drawContour{xshift=11.2cm,yshift=0}{diskEigExErrt1p0}{$E_x$-err}{$p$}{$t=1.0$}{$-7.8e-8$}{$7.8e-8$};
% 
% grid:
  % \draw[step=1cm,gray] (1,0) grid (17,5.6);
\end{tikzpicture}
}% end resize box
\end{center}
\caption{ MLA4 disk, GDM layer 1, ISO layer 2, vacuum outer domain. Modulated Gaussian plane wave. $\| \Ev\|$
   }
  \label{fig:oneDiskTwoLayersEfiledNormS22}
\end{figure}
}



==> tex/timeStep.tex <==
% =====================================================================
\newcommand{\CFL}{C_{\rm cfl}}
\subsection{Choosing the time-step} \label{sec:timeStep}

In this section we describe how the time-step $\dt$ is chosen.
%
First consider the case of the isotropic Maxwell's equations with no dispersive or nonlinear effects. 
On a Cartesian grid the time-step for the second-order accurate or fourth-order accurate scheme
is chosen from 
\ba
    c^2 \dt^2 \left[ \sum_{m=1}^{\nd} \f{1}{\dx_m^2} \right] = \CFL  \label{eq:timeStepMaxwell}
\ea
It can be shown from von Neumann stability analysis that the schemes are stable up to $\CFL=1$ and we choose $\CFL=.9$ by default.
On a curvilinear grid the coefficients in the discretization of Maxwell's equations will depend on space.
To choose the time-step in this case we freeze the coefficients and perform a von Neumann analysis on the 
frozen coefficient problems. This gives a time-step $\dt_\jv$ at each grid point. 
The time-step is then chosen as the minimum of $\dt_\jv$ over all grid points.

% The time-step chosen in this way can often be used for the full Maxwell-MLA equations since the additional terms
% will only contribute 

As explained in~\cite{adegdm2019} for the dispersive Maxwell equations,
the time-step for the full Maxwell-MLA equations will be a small perturbation to the
time-step determined for isotropic Maxwell's equations as the mesh spacing goes to zero. However, depending on the
size of the grid spacing (e.g. a coarse grid), the 
size of the coefficients in the MLA approximations, and the size of the nonlinear terms, it may be necessary to 
determine a more careful estimate for the time-step. Due to the nonlinear terms the maximum stable time-step will
depend on the current solution state.


A stable time-step for the full Maxwell-MLA equations can be found by linearizing the discrete equations about
some current state $\Qv^{(0)}=[\Ev^{(0)},\Pv^{(0)},\Nv^{(0)}]$. 
The time-step for the linearized equations is found by freezing coefficients and
performing a von Neumann analysis on the resulting linear equations. 


